AGB Variables and the Mira Period-Luminosity Relation

Published data for large amplitude asymptotic giant branch variables in the Large Magellanic Cloud are re-analysed to establish the constants for an infrared (K) period-luminosity relation of the form: Mk=rho[log P-2.38] + delta. A slope of rho=-3.51+/-0.20 and a zero point of delta=-7.15+/-0.06 are found for oxygen-rich Miras (if a distance modulus of 18.39+/-0.05 is used for the LMC). Assuming this slope is applicable to Galactic Miras we discuss the zero-point for these stars using the revised Hipparcos parallaxes together with published VLBI parallaxes for OH Masers and Miras in Globular Clusters. These result in a mean zero-point of delta=-7.25+/-0.07 for O-rich Galactic Miras. The zero-point for Miras in the Galactic Bulge is not significantly different from this value. Carbon-rich stars are also discussed and provide results that are consistent with the above numbers, but with higher uncertainties. Within the uncertainties there is no evidence for a significant difference between the period-luminosity relation zero-points for systems with different metallicity.

==> data.tex <==
 W Psc 
   JD     &   $J$ &   $H$ &   $K$ & $L$  \\
-2440000  &       &       &       &  \\
  9356.26 &  6.91 &  6.01 &  5.69 &  5.34\\
 10053.29 &  6.96 &  6.02 &  5.69 &  5.24\\
 10295.64 &  6.92 &  6.01 &  5.65 &  5.26\\
 10320.57 &  7.22 &  6.33 &  5.93 &  5.44\\
 10360.46 &  7.44 &  6.57 &  6.14 &  5.80\\
 10414.31 &  7.28 &  6.41 &  6.08 &  5.52\\
 10721.47 &  7.34 &  6.47 &  6.05 &  5.69\\
 10796.28 &  7.13 &  6.21 &  5.89 &  5.38\\
 11068.27 &  7.13 &  6.22 &  5.83 &  5.41\\
 11104.27 &  7.47 &  6.58 &  6.16 &  5.72\\
 12977.29 &  7.55 &  6.66 &  6.24 &  5.77\\
 WW Vel
 10792.54 &  4.15 &  3.05 &  2.51 &  1.91\\
 10848.51 &  4.12 &  3.08 &  2.54 &  1.87\\
 10917.40 &  3.81 &  2.88 &  2.41 &  1.81\\
 10949.48 &  3.78 &  2.84 &  2.40 &  1.85\\
 11864.60 &  3.22 &  2.22 &  1.83 &  1.38\\
 11883.59 &  3.30 &  2.29 &  1.86 &  1.42\\
 11965.48 &  3.97 &  2.88 &  2.35 &  1.81\\
 11976.47 &  4.08 &  2.97 &  2.43 &  1.86\\
 12069.26 &  4.07 &  3.05 &  2.52 &  1.88\\
 12087.24 &  4.01 &  3.03 &  2.51 &  1.87\\
 12116.19 &  3.95 &  2.98 &  2.50 &  1.87\\
 12243.57 &  3.28 &  2.29 &  1.91 &  1.45\\
 12257.61 &  3.29 &  2.29 &  1.89 &  1.43\\
 12287.56 &  3.39 &  2.35 &  1.92 &  1.46\\
 12319.53 &  3.58 &  2.52 &  2.05 &  1.62\\
 12347.46 &  3.78 &  2.68 &  2.19 &  1.73\\
 12382.38 &  4.02 &  2.87 &  2.35 &  1.87\\
 12426.26 &  3.98 &  2.91 &  2.39 &  1.87\\
 12456.24 &  3.84 &  2.82 &  2.34 &  1.80\\
 12661.60 &  3.27 &  2.24 &  1.83 &  1.42\\
 12664.53 &  3.27 &  2.25 &  1.84 &  1.43\\
 12691.53 &  3.39 &  2.34 &  1.91 &  1.49\\
 12755.34 &  3.94 &  2.82 &  2.30 &  1.79\\
 12825.24 &  4.17 &  3.07 &  2.52 &  1.94\\
 13031.58 &  3.26 &  2.26 &  1.89 &  1.46\\
 13060.51 &  3.30 &  2.27 &  1.87 &  1.46\\
 13118.37 &  3.61 &  2.53 &  2.06 &  1.59\\
 13137.29 &  3.81 &  2.71 &  2.20 &  1.72\\
 13172.28 &  4.10 &  2.98 &  2.43 &  1.87\\
 13205.22 &  4.11 &  3.02 &  2.47 &  1.93\\
 13405.57 &  3.36 &  2.37 &  2.00 &  1.58\\
 13415.46 &  3.29 &  2.31 &  1.94 &  1.50\\
 13434.57 &  3.24 &  2.25 &  1.86 &  1.45\\
 13454.45 &  3.27 &  2.23 &  1.84 &  1.42\\
 13508.30 &  3.55 &  2.49 &  2.01 &  1.60\\
 13560.21 &  4.01 &  2.90 &  2.38 &  1.86\\
 13935.20 &  4.05 &  2.94 &  2.38 &  1.86\\
 14140.52 &  3.76 &  2.82 &  2.37 &  1.83\\
 RT Crt
 10792.59 &  5.75 &  4.96 &  4.48 &  3.75\\
 10848.61 &  5.42 &  4.57 &  4.13 &  3.49\\
 10948.74 &  6.20 &  5.37 &  4.85 &  4.11\\
 11966.49 &  5.44 &  4.61 &  4.20 &  3.68\\
 11979.43 &  5.57 &  4.74 &  4.30 &  3.80\\
 12257.59 &  5.98 &  5.28 &  4.85 &  4.15\\
 12319.55 &  5.60 &  4.76 &  4.37 &  3.87\\
 12349.44 &  5.87 &  5.04 &  4.61 &  4.10\\
 12383.36 &  6.47 &  5.61 &  5.05 &  4.41\\
 12425.29 &  6.34 &  5.49 &  4.96 &  4.24\\
 12457.23 &  5.63 &  4.82 &  4.46 &  3.85\\
 12695.49 &  5.46 &  4.58 &  4.16 &  3.59\\
 13065.41 &  5.42 &  4.59 &  4.19 &  3.70\\
 13139.34 &  6.37 &  5.54 &  4.96 &  4.37\\
 13454.43 &  5.68 &  4.82 &  4.38 &  3.84\\
 13906.25 &  6.25 &  5.38 &  4.82 &  4.12\\
 S CrB 
 10528.02 &  1.40 &  0.46 &  0.00 & -0.46\\
 10564.50 &  1.71 &  0.77 &  0.22 & -0.26\\
 10948.31 &  1.82 &  0.88 &  0.33 & -0.26\\
 10980.31 &  1.96 &  1.02 &  0.43 & -0.21\\
 12800.37 &  2.12 &  1.16 &  0.55 & -0.08\\
 13454.56 &  1.75 &  0.78 &  0.26 & -0.25\\
 13506.44 &  2.08 &  1.08 &  0.49 & -0.07\\
 13563.29 &  2.07 &  1.10 &  0.51 & -0.14\\
 S Ser 
 10528.63 &  3.01 &  2.08 &  1.60 &  1.00\\
 10564.51 &  3.05 &  2.10 &  1.62 &  1.03\\
 10947.14 &  3.44 &  2.51 &  2.00 &  1.37\\
 10997.28 &  2.88 &  2.01 &  1.61 &  1.11\\
 12800.36 &  3.37 &  2.40 &  1.88 &  1.25\\
 13434.61 &  3.78 &  2.63 &  2.06 &  1.45\\
 13444.63 &  3.73 &  2.63 &  2.01 &  1.48\\
 13454.58 &  3.66 &  2.57 &  1.99 &  1.44\\
 13506.42 &  3.29 &  2.32 &  1.81 &  1.24\\
 13563.29 &  3.33 &  2.37 &  1.87 &  1.29\\
 BG Ser
 10946.14 &  2.10 &  0.94 &  0.45 &  0.02\\
 10997.27 &  2.15 &  1.06 &  0.55 &  0.07\\
 11053.14 &  1.92 &  0.91 &  0.48 &  0.03\\
 13412.64 &  1.89 &  0.84 &  0.40 & -0.06\\
 13434.63 &  1.93 &  0.88 &  0.44 & -0.02\\
 13454.63 &  1.89 &  0.83 &  0.40 & -0.03\\
 13506.47 &  1.82 &  0.74 &  0.33 & -0.07\\
 13558.36 &  1.75 &  0.64 &  0.23 & -0.14\\
 R Ser 
  2547.00 &  2.10 &  1.24 &  0.67 &  0.07\\
  2862.00 &  2.31 &  1.44 &  0.90 &  0.30\\
  2951.00 &  2.52 &  1.65 &  1.12 &  0.38\\
  2974.00 &  2.45 &  1.57 &  1.08 &  0.30\\
  3216.00 &  2.03 &  1.06 &  0.52 & -0.01\\
  3238.00 &  2.10 &  1.14 &  0.62 & -0.06\\
 12755.52 &  1.64 &  0.70 &  0.24 & -0.22\\
 12800.39 &  2.02 &  1.07 &  0.55 &  0.04\\
 12832.32 &  2.20 &  1.20 &  0.67 &  0.13\\
 13438.64 &  1.46 &  0.54 &  0.11 & -0.37\\
 13454.60 &  1.57 &  0.60 &  0.21 & -0.25\\
 13506.46 &  1.95 &  0.98 &  0.53 &  0.04\\
 13558.36 &  2.14 &  1.16 &  0.68 &  0.17\\
 RU Her
 10528.63 &  2.24 &  1.02 &  0.42 & -0.15\\
 10564.34 &  2.42 &  1.19 &  0.55 &  0.00\\
 10948.25 &  1.64 &  0.51 &  0.01 & -0.45\\
 10997.32 &  1.96 &  0.79 &  0.21 & -0.31\\
 12800.40 &  1.50 &  0.51 &  0.07 & -0.48\\
 13444.64 &  2.14 &  0.98 &  0.40 & -0.10\\
 13454.63 &  2.25 &  1.06 &  0.47 & -0.06\\
 13506.47 &  2.65 &  1.39 &  0.74 &  0.10\\
 13563.31 &  2.31 &  1.20 &  0.60 & -0.06\\
 T Her 
 10565.60 &  4.54 &  3.83 &  3.55 &  3.07\\
 10948.31 &  4.38 &  3.51 &  3.14 &  2.75\\
 11052.31 &  4.45 &  3.57 &  3.25 &  2.80\\
 13454.65 &  4.65 &  3.77 &  3.35 &  2.92\\
 W Sex 
 10948.20 &  5.18 &  4.00 &  3.51 &  3.06\\
 11890.60 &  5.00 &  3.85 &  3.42 &  2.97\\
 11963.43 &  5.36 &  4.16 &  3.61 &  3.13\\
 11979.42 &  5.07 &  3.94 &  3.49 &  3.05\\
 12257.55 &  5.03 &  3.88 &  3.44 &  3.04\\
 12287.52 &  5.06 &  3.91 &  3.45 &  2.99\\
 12319.48 &  5.08 &  3.94 &  3.48 &  3.06\\
 12347.43 &  5.44 &  4.20 &  3.64 &  3.19\\
 12383.35 &  5.20 &  4.03 &  3.55 &  3.13\\
 12425.28 &  4.94 &  3.85 &  3.43 &  3.06\\
 12457.20 &  5.08 &  3.92 &  3.50 &  3.09\\
 12664.51 &  5.03 &  3.89 &  3.45 &  3.05\\
 12693.47 &  5.12 &  3.94 &  3.47 &  3.04\\
 12801.23 &  4.98 &  3.86 &  3.45 &  3.04\\
 13029.53 &  4.88 &  3.78 &  3.39 &  2.98\\
 13063.45 &  4.98 &  3.83 &  3.41 &  2.96\\
 13438.49 &  4.90 &  3.80 &  3.40 &  2.99\\
 13906.21 &  5.01 &  3.86 &  3.42 &  2.97\\
 14140.51 &  5.09 &  3.93 &  3.46 &  3.03\\

